Real Time Bearing Fault Diagnosis Based on Convolutional Neural Network and STM32 Microcontroller

With the rapid development of big data and edge computing, many researchers focus on improving the accuracy of bearing fault classification using deep learning models, and implementing the deep learning classification model on limited resource platforms such as STM32. To this end, this paper realizes the identification of bearing fault vibration signal based on convolutional neural network, the fault identification accuracy of the optimised model can reach 98.9%. In addition, this paper successfully applies the convolutional neural network model to STM32H743VI microcontroller, the running time of each diagnosis is 19ms. Finally, a complete real-time communication framework between the host computer and the STM32 is designed, which can perfectly complete the data transmission through the serial port and display the diagnosis results on the TFT-LCD screen.

==> Real_Time_Bearing_Fault_Diagnosis_Based_on_Convolutional_Neural_Network_and_STM32_Microcontroller <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{1}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{leiApplicationsMachineLearning2020}
Y.~Lei, B.~Yang, X.~Jiang, F.~Jia, N.~Li, and A.~K. Nandi, ``Applications of
  machine learning to machine fault diagnosis: {{A}} review and roadmap,''
  \emph{Mechanical Systems and Signal Processing}, vol. 138, p. 106587, Apr.
  2020.

\bibitem{zhaoDeepResidualShrinkage2020}
M.~Zhao, S.~Zhong, X.~Fu, B.~Tang, and M.~Pecht, ``Deep {{Residual Shrinkage
  Networks}} for {{Fault Diagnosis}},'' \emph{IEEE Transactions on Industrial
  Informatics}, vol.~16, no.~7, pp. 4681--4690, Jul. 2020.

\bibitem{BearingDataCenter2021}
``Bearing {{Data Center}} | {{Case School}} of {{Engineering}} | {{Case Western
  Reserve University}},'' https://engineering.case.edu/bearingdatacenter, Aug.
  2021.

\bibitem{boudiafComparativeStudyVarious2016}
A.~Boudiaf, A.~Moussaoui, A.~Dahane, and I.~Atoui, ``A {{Comparative Study}} of
  {{Various Methods}} of {{Bearing Faults Diagnosis Using}} the {{Case Western
  Reserve University Data}},'' \emph{Journal of Failure Analysis and
  Prevention}, vol.~16, no.~2, pp. 271--284, Apr. 2016.

\bibitem{smithRollingElementBearing2015}
W.~A. Smith and R.~B. Randall, ``Rolling element bearing diagnostics using the
  {{Case Western Reserve University}} data: {{A}} benchmark study,''
  \emph{Mechanical Systems and Signal Processing}, vol. 64--65, pp. 100--131,
  Dec. 2015.

\bibitem{refwuJiyujuanjishenjingwangluodejixieguzhangzhenduanfangfazongshu2020}
D.~Wu, G.~Ren, H.~Wang, and Y.~Zhang, ``{A Survey of Mechanical Fault Diagnosis
  Methods Based on Convolutional Neural Networks},'' \emph{Journal of
  Mechanical Strength}, vol.~42, no.~05, pp. 1024--1032, 2020.

\bibitem{XCUBEAIAIExpansion}
``X-{{CUBE-AI}} - {{AI}} expansion pack for {{STM32CubeMX}} -
  {{STMicroelectronics}},''
  https://www.st.com/en/embedded-software/x-cube-ai.html.

\end{thebibliography}

